Strategic programming on graph rewriting systems

We describe a strategy language to control the application of graph rewriting rules, and show how this language can be used to write high-level declarative programs in several application areas. This language is part of a graph-based programming tool built within the port-graph transformation and visualisation environment PORGY.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{H. Kirchner, C. Mu\~noz (Eds.): First International Workshop on\\ Strategies in Rewriting, Proving, and Programming (IWS 2010)\\
EPTCS 44, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.44.1}{10.4204/EPTCS.44.1}}
\pdfoutput=1

